Barbara Rokowska's combinatorial research with her extensive biography (1926--2012)

We discuss the significance of some interesting results by Barbara Rokowska about combinatorial constructions. Her interest in finite mathematics and number theory began with an embellishment and detailing of some work by Erdos. Rokowska and Schinzel then solved the problem posed by Paul Erdos concerning the existence of prime numbers of a certain kind. Her subsequent work highlighted the difficulty in constructing Steiner systems with certain properties and showed the importance of rigorous proof techniques in this area of mathematics. This is the first such summary of the main results obtained by Rokowska, her collaborators and PhD students. A biography of Barbara Rokowska has been added as an appendix.

==> Parts/AMv18BRokowska17x2024bib.tex <==
%% Bibliografia


%%%%%%%%%%%%%%%%%%%%%%%%%%

==> arXiv/AMv17BFLysikKSz20viii23bib.tex <==
%% Bibliografia


%%%%%%%%%%%%%%%%%%%%%%%%%%

==> arXiv/AMv18BRokowska16x2024bib.tex <==
%% Bibliografia


%%%%%%%%%%%%%%%%%%%%%%%%%%

==> arXiv/AMv18BRokowska25ix2024bib.tex <==
%% Bibliografia


%%%%%%%%%%%%%%%%%%%%%%%%%%
